HDR-Plenoxels: Self-Calibrating High Dynamic Range Radiance Fields

We propose high dynamic range (HDR) radiance fields, HDR-Plenoxels, that learn a plenoptic function of 3D HDR radiance fields, geometry information, and varying camera settings inherent in 2D low dynamic range (LDR) images. Our voxel-based volume rendering pipeline reconstructs HDR radiance fields with only multi-view LDR images taken from varying camera settings in an end-to-end manner and has a fast convergence speed. To deal with various cameras in real-world scenarios, we introduce a tone mapping module that models the digital in-camera imaging pipeline (ISP) and disentangles radiometric settings. Our tone mapping module allows us to render by controlling the radiometric settings of each novel view. Finally, we build a multi-view dataset with varying camera conditions, which fits our problem setting. Our experiments show that HDR-Plenoxels can express detail and high-quality HDR novel views from only LDR images with various cameras.

==> figure/tex/ablation_study_1.tex <==

\begin{table}
    \centering
    \caption{
    \textbf{Analysis on initialization on harsh setting.}
    Learning with a saturation mask alone cannot guarantee performance in a harsh condition with a high saturation ratio.
    Initialization helps our model to maintain its performance robust to the input condition.
    }
    \resizebox{0.75\textwidth}{!}{ 
        \begin{tabular}{l@{\quad}cc@{\quad}ccc}
        \toprule
        \textbf{Index} & \textbf{Sat} & \textbf{Init} & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$  \\
        \midrule
        w/o init, sat & $\times$ & $\times$ & $28.58$ & $0.889$ & $0.306$ \\
        w/ sat & $\checkmark$ & $\times$ & $28.58$ & $0.889$ & $0.306$ \\
        w/ init & $\times$ & $\checkmark$ & \textbf{28.77} & \textbf{0.895} & \textbf{0.294} \\
        Ours (w/ init, sat) & $\checkmark$ & $\checkmark$ & $28.76$ & \textbf{0.895} & \textbf{0.294} \\
        % w/o init, sat & $\times$ & $\times$ & $28.5770$ & $0.8891$ & $0.3061$ \\
        % w/ sat & $\checkmark$ & $\times$ & $28.5760$ & $0.8891$ & $0.3061$ \\
        % w/ init & $\times$ & $\checkmark$ & \textbf{28.7656} & \textbf{0.8945} & \textbf{0.2943} \\
        % Ours (w/ init, sat) & $\checkmark$ & $\checkmark$ & $28.7552$ & $0.8945$ & $0.2941$ \\
        \bottomrule
        \end{tabular}
    }
    \label{table:ablation_1}
\end{table}


==> figure/tex/nn_result.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
%   \vspace{-8mm}
  \centering
  \includegraphics[width=0.48\textwidth]{figure/nn_result.pdf}
%   \vspace{-3mm}
  \caption{\textbf{Implicit CRF model result}.}
%   \vspace{-8mm}
\end{wrapfigure}

==> figure/tex/quan_average.tex <==
%% syn llff 평균

\begin{table}
    \centering
    \caption{Font sizes of headings. Table captions should always be
    positioned {\it above} the tables. The final sentence of a table
    caption should end without a full stop}
    \resizebox{0.7\textwidth}{!}{ 
        \begin{tabular}{@{\quad}l@{\quad}ccc@{\quad}ccc@{\ }}
        \toprule
        \multirow{2}[2]{*}{\textbf{Method}}& \multicolumn{3}{c}{\textbf{Blender Synthetic}} & \multicolumn{3}{c}{\textbf{Real Data}} \\
        \cmidrule(r{10pt}){2-4} \cmidrule(r{3pt}){5-7}
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ \\
        \midrule
         Mid 
         & $27.99$ & $0.868$ & $0.277$
         & $27.45$ & $0.905$ & $0.311$ \\
         Mix
         & $13.74$ & $0.561$ & $0.607$ 
         & $15.37$ & $0.592$ & $0.520$  \\
         Ours
         & $28.18$ & $0.874$ & $0.302$ 
         & $29.98$ & $0.917$ & $0.305$  \\
         ADOP
         & - & - & -
         & - & - & - \\
         NeRF-W
         & - & - & -
         & - & - & - \\
        %  Mid 
        %  & $27.9896$ & $0.8681$ & $0.2770$
        %  & $27.4455$ & $0.9052$ & $0.3110$ \\
        %  Mix
        %  & $13.7352$ & $0.5606$ & $0.6066$ 
        %  & $15.3680$ & $0.5923$ & $0.5203$  \\
        %  Ours
        %  & $28.1800$ & $0.8739$ & $0.3024$ 
        %  & $29.9780$ & $0.9168$ & $0.3045$  \\
         \bottomrule
        \end{tabular}}
    \label{table:quan_average}
\end{table}

==> figure/tex/quan_real.tex <==
%% real data 항목마다


\begin{table}
    \centering
    \caption{Font sizes of headings. Table captions should always be
    positioned {\it above} the tables. The final sentence of a table
    caption should end without a full stop}
    \resizebox{0.7\textwidth}{!}{ 
        \begin{tabular}{@{\quad}l@{\quad}ccc@{\quad}ccc@{\ }}
        \toprule
        \multirow{2}[2]{*}{\textbf{Method}}& \multicolumn{3}{c}{\textbf{Bright Desk}} & \multicolumn{3}{c}{\textbf{Dark Desk}} \\
        \cmidrule(r{10pt}){2-4} \cmidrule(r{3pt}){5-7}
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ \\
        \midrule
         Mid 
         & $29.37$ & $0.916$ & $0.319$
         & $25.53$ & $0.895$ & $0.303$ \\
         Mix
         & $16.99$ & $0.632$ & $0.523$ 
         & $13.75$ & $0.553$ & $0.518$ \\
         Ours
         & $30.79$ & $0.916$ & $0.312$ 
         & $29.17$ & $0.918$ & $0.297$ \\
         ADOP
         & - & - & -
         & - & - & - \\
         NeRF-W
         & - & - & -
         & - & - & - \\
        %  Mid 
        %  & $29.3660$ & $0.9159$ & $0.3193$
        %  & $25.5250$ & $0.8945$ & $0.3027$ \\
        %  Mix
        %  & $16.9890$ & $0.6321$ & $	0.5227$ 
        %  & $13.7470$ & $0.5526$ & $	0.5178$ \\
        %  Ours
        %  & $30.7880$ & $0.9159$ & $	0.3119$ 
        %  & $29.1680$ & $0.9176$ & $	0.2971$ \\
         \bottomrule
        \end{tabular}}
    \label{table:quan_real}
\end{table}





==> figure/tex/quan_real_average.tex <==
%% syn llff 평균

% \begin{table}
\begin{wraptable}{r}{0.5\linewidth}
    \centering
    % \vspace{-8mm}
    \caption{\textbf{Quantitative comparison on real data.} Results are averaged over the 2 real scenes. $\mathcal{S}$ denote the static and $\mathcal{D}$ is the dynamic datasets.
    % \vspace{-3mm}
    }
    \resizebox{0.95\linewidth}{!}
    { 
    \begin{tabular}{@{}c@{\quad}l@{\quad}c@{\quad}c@{\quad}c}
        \toprule 
         \multirow{2}[2]{*}{\textbf{Type}} & \multirow{2}[2]{*}{\textbf{Method}}& \multicolumn{3}{c}{\textbf{Real Data}} \\
         \cmidrule(r){3-5}
          & & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ \\
         \midrule
        %  Static  & $27.4455$ & $0.9052$ & $0.3110$ \\
        %  Dynamic  & $15.3680$ & $0.5923$ & $0.5203$ \\
        %  Dynamic w\ ours & $29.9780$ & $0.9168$ & $0.3045$ \\
         $\mathcal{S}$ 
          & Baseline & $27.45$ & $0.905$ & $0.311$ \\
         \cmidrule{1-5}
         \multirow{4}{*}{$\mathcal{D}$} 
          & Baseline & $15.37$ & $0.592$ & $0.520$ \\
          & ADOP     & - & - & - \\
          & NeRF-W   & - & - & - \\
          & Ours     & $29.98$ & $0.917$ & $0.305$ \\
        \bottomrule
    \end{tabular}}
    \label{table:quan_real_average}
    % \vspace{-7mm}
\end{wraptable}
% \end{table}


==> figure/tex/quan_syn_before.tex <==
%% syn llff 평균
\begin{table}[t]
    \centering
    % \vspace{-5mm}
    \caption{\textbf{Quatitative results of novel view synthesis on synthetic data.}
    Values are average of the results for the test data of each scene.
    For evaluation, ADOP exploits all the input images as it needs dense reconstruction.
    For the other models, the left half of the image was included in the learning data and learned, and tested on the unseen right half of the image.
    Our model shows overall high performance compared to other models.
    $\mathcal{S}$ denote the static and $\mathcal{V}$ is the varying datasets.
    The \textbf{\green{green}} color and the \textbf{\blue{blue}} color stand for the best and the second best, respectively.
    }
    \resizebox{\textwidth}{!}{ 
        \begin{tabular}{c@{\ }l@{\ }ccc@{\ }ccc@{\ }ccc@{\ }ccc@{\ }ccc}
        \toprule
         \multirow{2}[2]{*}{\textbf{Type}} & \multirow{2}[2]{*}{\textbf{Method}}
         & \multicolumn{3}{c}{\textbf{Book}}
         & \multicolumn{3}{c}{\textbf{Classroom}}
         & \multicolumn{3}{c}{\textbf{Monk}}
         & \multicolumn{3}{c}{\textbf{Room}} 
         & \multicolumn{3}{c}{\textbf{Kitchen}} \\
         \cmidrule(rl){3-5} \cmidrule(rl){6-8} \cmidrule(rl){9-11} \cmidrule(rl){12-14} \cmidrule(rl){15-17}
         && \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ \\
        \midrule
         $\mathcal{S}$ & Baseline 
         & 22.60 & 0.803 & 0.309 
         & 27.02 & 0.872 & 0.324 
         & 26.77 & 0.816 & 0.352 
         & 30.05 & 0.897 & 0.234 
         & 33.52 & 0.953 & 0.166 
         \\
         \cmidrule{1-17}
         \multirow{4}{*}{$\mathcal{V}$} & Baseline
         & 12.12 & 0.447 & 0.618 
         & 12.98 & 0.528 & 0.676 
         & 12.22 & 0.532 & 0.568 
         & 12.85 & 0.580 & 0.665 
         & 18.52 & 0.717 & 0.507 
        \\
         & ADOP
         & \textbf{\blue{20.92}} & 0.820 & \textbf{\green{0.194}} 
         & \textbf{\blue{23.33}} & \textbf{\green{0.885}} & \textbf{\green{0.154}} 
         & \textbf{\blue{23.86}} & \textbf{\green{0.861}} & \textbf{\green{0.124}} 
         & \textbf{\blue{24.74}} & \textbf{\green{0.909}} & \textbf{\green{0.113}} 
         & \textbf{\blue{27.67}} & \textbf{\green{0.952}} & \textbf{\green{0.083}}
        \\
         & NeRF-W
         & 15.06 & \textbf{\blue{0.840}} & 0.490 
         & 13.84 & 0.660 & 0.630 
         & 11.95 & 0.500 & 0.690 
         & 11.55 & 0.680 & 0.740 
         & 18.92 & 0.790 & 0.490 
         \\
        & Ours
         & \textbf{\green{27.57}} & \textbf{\green{0.845}} & \textbf{\blue{0.294}} 
         & \textbf{\green{28.25}} & \textbf{\blue{0.883}} & \textbf{\blue{0.343}} 
         & \textbf{\green{27.28}} & \textbf{\blue{0.820}} & \textbf{\blue{0.369}} 
         & \textbf{\green{26.23}} & \textbf{\blue{0.887}} & \textbf{\blue{0.339}} 
         & \textbf{\green{31.58}} & \textbf{\blue{0.935}} & \textbf{\blue{0.166}} \\
        %  Static 
        %  & $22.5960$ & $0.8034$ & $0.3090$ 
        %  & $27.0150$ & $0.8720$ & $0.3242$ 
        %  & $26.7740$ & $0.8161$ & $0.3521$ 
        %  & $30.0460$ & $0.8966$ & $0.2339$ 
        %  & $33.5170$ & $0.9526$ & $0.1657$
        % \\
        %  $ $
        %  Dynamic
        %  & $12.1160$ & $0.4470$ & $0.6181$ 
        %  & $12.9750$ & $0.5280$ & $0.6756$ 
        %  & $12.2160$ & $0.5317$ & $0.5676$ 
        %  & $12.8520$ & $0.5797$ & $0.6647$ 
        %  & $18.5170$ & $0.7165$ & $0.5072$
        
        % \\
        %  $ $ 
        %  Dynamic w/ ours
        %  & $27.5660$ & $0.8451$ & $0.2942$ 
        %  & $28.2480$ & $0.8826$ & $0.3432$ 
        %  & $27.2780$ & $0.8197$ & $0.3694$ 
        %  & $26.2290$ & $0.8873$ & $0.3391$ 
        %  & $31.5790$ & $0.9348$ & $0.1663$
        % \\
        % & ADOP
        %  & $20.9176$ & $0.819586$ & $0.193668$ 
        %  & $23.3283$ & $0.885339$ & $0.153619$ 
        %  & $23.8649$ & $0.861316$ & $0.124225$ 
        %  & $24.7399$ & $0.909442$ & $0.112928$ 
        %  & $27.6746$ & $0.951607$ & $0.0834881$
         \bottomrule
        \end{tabular}
    }
    \label{table:quan_syn}
    % \vspace{-5mm}
\end{table}

==> figure/tex/save.tex <==
% \begin{figure}
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figure/saturation/sat_dark.pdf}
%         \caption{}
%     \end{subfigure}
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{figure/saturation/sat_bright.pdf}
%         \caption{}
%     \end{subfigure}
%     \caption{\textbf{Saturation mask.} Saturation mask at red, green, and blue sequentially.}
%     \label{fig:sat_mask}
%     \vspace{-6mm}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \rotatebox[origin=c]{90}{$book$}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \\ 
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \rotatebox[origin=c]{90}{$book$}
%         {
%             \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%             \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%         }{Ours}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         {
%             \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%             \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%         }{Ours}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         {
%             \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%             \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%         }{Ours}
%     \end{subfigure}%
%     \footnotesize
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         {
%             \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%             \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%         }{Ours}
%     \end{subfigure}%
%     \caption{\textbf{Qualitative comparison of other baselines.} There are the comparsion of novel LDR rendering with training a multi exposure.}
%     \label{fig:sat_mask}
%     \vspace{-6mm}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \rotatebox[origin=c]{90}{$book$}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \\ 
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \rotatebox[origin=c]{90}{$book$}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \begin{subfigure}[b]{0.25\textwidth}
%         \centering
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_ldr.png}\hspace{-0.7mm}
%         \includegraphics[width=0.4\textwidth]{figure/qual_baseline/ours_mse.png}
%     \end{subfigure}%
%     \caption{\textbf{Qualitative comparison of other baselines.} There are the comparsion of novel LDR rendering with training a multi exposure.}
%     \label{fig:sat_mask}
%     \vspace{-6mm}
% \end{figure}

==> rebuttal_figure/tex/shot_noise.tex <==
% \begin{wraptable}{r}{0.48\linewidth}
% % \caption{.}
% % \label{wrap-tab:1}
% \begin{tabular}{cccc}\\\toprule
% \hline
%  & PSNR & SSIM & LPIPS \\
% \hline
% w/ noise & 28.27 & 0.894 & 0.274 \\
% w/o noise & 29.53 & 0.918 & 0.166 \\
% \hline
% \end{tabular}
% \end{wraptable} 

% \begin{table}[ht]
% \begin{tabular}{cccc}\\\toprule
% \hline
%  & PSNR & SSIM & LPIPS \\
% \hline
% w/ noise & 28.27 & 0.894 & 0.274 \\
% w/o noise & 29.53 & 0.918 & 0.166 \\
% \hline
% \end{tabular}
% \end{table}

\begin{table}[ht]
\caption{
    \textbf{Title.}
    Explanation.
    }
    \resizebox{0.45\textwidth}{!}{ 
    \centering
    \begin{tabular}{cccc}\\\toprule
     & PSNR & SSIM & LPIPS \\
    \hline
    w/ noise & 28.27 & 0.894 & 0.274 \\
    w/o noise & 29.53 & 0.918 & 0.166 \\
    \hline
    \end{tabular}}
\end{table}


==> supple_figure/ftex/qual_baseline.tex <==
\begin{figure}[t]
\setlength{\abovecaptionskip}{0mm} 
    \centering
    \includegraphics[width=1\linewidth]{supple_figure/sup_baseline.pdf}
    % \vspace{-7mm}
    \caption{\textbf{Comparisons of qualitative results to baseline.}
    The first row represents the LDR reference image, which is used at training.
    All experiments are trained with varying conditioned data and rendered with tone mapping stage.
    Our results represent fine-grained rendering results compared to the ADOP baseline.
    Especially, ours shows satisfying color representations compared to ADOP.
    }
    \label{sup_fig:baseline}
    % \vspace{-3mm}
\end{figure}

==> supple_figure/ftex/qual_crf_rgb.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{supple_figure/crf_rgb.pdf}
    % \vspace{-7mm}
    \caption{\textbf{CRF according to color channels.}
    There are comparisons of CRF function at each color channel between standard and filmic transforms.}
    \label{sup_fig:crf_rgb}
    % \vspace{-5mm}
\end{figure}

==> supple_figure/ftex/qual_denoise.tex <==
% \setlength{\columnsep}{5pt}%
\begin{wrapfigure}{r}{0.40\linewidth}
  \setlength{\abovecaptionskip}{-1mm}
  \centering
  \includegraphics[width=1\linewidth]{rebuttal_figure/shot_noise.pdf}
  \caption{\textbf{Denoising effect of HDR-Plenoxels.}}
    % Images show input kitchen data with shot noise (left) and qualitative result of our models trained on images with (middle) or without shot noise (right). Our model show denoising effects to some extent.
    % }
    \label{sup_fig:qual_denoise}
  % \setlength{\belowcaptionskip}{-10mm}
\end{wrapfigure}

==> supple_figure/ftex/qual_exp_change.tex <==
\begin{figure}[t]
\setlength{\abovecaptionskip}{-1mm}
    \centering
    \includegraphics[width=1\linewidth]{supple_figure/exp_change.pdf}
    % \vspace{-7mm}
    \caption{\textbf{Novel view synthesis results with varying exposure rendering.}
    The exposure condition changes from dark to bright from left to right.
    % There are novel view synthesis results of changing exposure from darker to lighter.
    The novel view rendering result of the middle column has a basis exposure value.
    % The middle is novel view rendering with basis exposure value.
    }
    \label{sup_fig:exp_change}
    % \vspace{-5mm}
\end{figure}

==> supple_figure/ftex/qual_wb_change.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{supple_figure/wb_change.pdf}
    % \vspace{-8mm}
    \caption{\textbf{Novel view synthesis results with varying white balance rendering.}
    % There are novel view synthesis results of changing the white balance among red, green, and blue.
    The white balance changes \wrt red, green, and blue, in the results of the second, third, and last columns, respectively.
    The novel view rendering result of the first column has a basis white balance value.
    % The left is novel view rendering with basis white balance value.
    }
    \label{sup_fig:wb_change}
    % \vspace{-3mm}
\end{figure}

==> supple_figure/ftex/quan_real_all.tex <==
%% syn llff 평균
\begin{table}[t]
\setlength{\belowcaptionskip}{1mm}
    \centering
    % \vspace{-5mm}
     \caption{\textbf{Quantitative results of novel view synthesis on real scenes.}
    % Values are average of the results for the test data of each scene.
    $\mathcal{S}$ denote the static and $\mathcal{V}$ is the varying datasets.
    The blue and red color stand for the \textbf{\rred{best}} and the \textbf{\blue{second best}}, respectively.
    We report the averaged results of all the views in each test data. 
    % Our method shows overall high performance compared to other models.
    Our method shows the highest or the second-best performance compared to other models.
    % \vspace{-3mm}
    }
    \resizebox{\textwidth}{!}{ 
        \begin{tabular}{c@{\ }l@{\ }ccc@{\ }ccc@{\ }ccc@{\ }ccc}
        \toprule
         \multirow{2}[2]{*}{\textbf{Type}} & \multirow{2}[2]{*}{\textbf{Method}}
        %  & \multicolumn{3}{c}{\textbf{Lamp}}
         & \multicolumn{3}{c}{\textbf{Character}}
         & \multicolumn{3}{c}{\textbf{Desk}}
         & \multicolumn{3}{c}{\textbf{Plant}} 
         & \multicolumn{3}{c}{\textbf{Coffee}} \\
         \cmidrule(rl){3-5} \cmidrule(rl){6-8} \cmidrule(rl){9-11} \cmidrule(rl){12-14} 
         &
        %  & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ 
         & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ \\
        \midrule
         $\mathcal{S}$ & Baseline 
        %  & 29.37 & 0.916 & 0.319
         & 32.40 & 0.955 & 0.278
         & 25.53 & 0.895 & 0.303
         & 24.58 & 0.833 & 0.324
         & 25.87 & 0.922 & 0.301
         \\
         \cmidrule{1-14}
         \multirow{3}{*}{$\mathcal{V}$} & Baseline
        %  & 16.99 & 0.632 & 0.523
         & \textbf{\blue{19.13}} & 0.762 & 0.526
         & \textbf{\blue{13.75}} & \textbf{\blue{0.553}} & \textbf{\blue{0.518}}
         & \textbf{\blue{21.29}} & \textbf{\blue{0.623}} & 0.511
         & 17.49 & 0.751 & 0.476
        \\
         & ADOP
        %  & \textbf{\blue{-}} & - & \textbf{\green{-}} 
         & 17.56 & \textbf{\blue{0.801}} & \textbf{\rred{0.114}} 
         & 10.298 & 0.390 & \textbf{\blue{0.518}}
         & 18.26 & 0.529 & \textbf{\rred{0.192}} 
         & \textbf{\blue{18.44}} & \textbf{\blue{0.822}} & \textbf{\rred{0.085}}
        % \\
        %  & NeRF-W
        %  & 15.06 & \textbf{\blue{0.840}} & 0.490 
        %  & 13.84 & 0.660 & 0.630 
        %  & 11.95 & 0.500 & 0.690 
        %  & 11.55 & 0.680 & 0.740 
        %  & 18.92 & 0.790 & 0.490 
         \\
         & Ours
        %  & \textbf{\green{30.60}} & \textbf{\green{0.917}} & \textbf{\blue{0.305}} 
         & \textbf{\rred{33.14}} & \textbf{\rred{0.960}} & \textbf{\blue{0.343}} 
         & \textbf{\rred{28.32}} & \textbf{\rred{0.907}} & \textbf{\rred{0.312}} 
         & \textbf{\rred{24.27}} & \textbf{\rred{0.790}} & \textbf{\blue{0.369}} 
         & \textbf{\rred{27.40}} & \textbf{\rred{0.928}} & \textbf{\blue{0.269}} 

         \\
        %  Static 
        %  & $22.5960$ & $0.8034$ & $0.3090$ 
        %  & $27.0150$ & $0.8720$ & $0.3242$ 
        %  & $26.7740$ & $0.8161$ & $0.3521$ 
        %  & $30.0460$ & $0.8966$ & $0.2339$ 
        %  & $33.5170$ & $0.9526$ & $0.1657$
        % \\
        %  $ $
        %  Dynamic
        %  & $12.1160$ & $0.4470$ & $0.6181$ 
        %  & $12.9750$ & $0.5280$ & $0.6756$ 
        %  & $12.2160$ & $0.5317$ & $0.5676$ 
        %  & $12.8520$ & $0.5797$ & $0.6647$ 
        %  & $18.5170$ & $0.7165$ & $0.5072$
        
        % \\
        %  $ $ 
        %  Dynamic w/ ours
        %  & $27.5660$ & $0.8451$ & $0.2942$ 
        %  & $28.2480$ & $0.8826$ & $0.3432$ 
        %  & $27.2780$ & $0.8197$ & $0.3694$ 
        %  & $26.2290$ & $0.8873$ & $0.3391$ 
        %  & $31.5790$ & $0.9348$ & $0.1663$
        % \\
        % & ADOP
        %  & $20.9176$ & $0.819586$ & $0.193668$ 
        %  & $23.3283$ & $0.885339$ & $0.153619$ 
        %  & $23.8649$ & $0.861316$ & $0.124225$ 
        %  & $24.7399$ & $0.909442$ & $0.112928$ 
        %  & $27.6746$ & $0.951607$ & $0.0834881$
         \bottomrule
        \end{tabular}
    }
    \label{sup_table:real_all}
    % \vspace{-5mm}
\end{table}





==> supple_figure/tex/qual_crf_rgb.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{supple_figure/crf_rgb.pdf}
    % \vspace{-7mm}
    \caption{\textbf{CRF according to color channels.}
    There are comparisons of CRF function at each color channel between standard and filmic transforms.}
    \label{sup_fig:crf_rgb}
    % \vspace{-5mm}
\end{figure}

==> supple_figure/tex/quan_extreme.tex <==
\begin{table}
\setlength{\abovecaptionskip}{2mm}
\setlength{\belowcaptionskip}{1mm}
    \centering
    \small
    \caption{\textbf{PSNR on extreme conditions.}}
    % We consider replacing the averaging in $\gs$ with either max-pooling or the class token. We show ImageNet-1K \ug{top-1 accuracy} on the validation set.}
    \label{table:hard}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{c CCCC}
         \toprule
          Exposure & $\pm$3EV & $\pm$4EV & $\pm$5EV & $\pm$6EV\\
         \midrule
         PSNR & $\ourpsnr$ & 30.30 & 29.10 & 28.48\\
         \bottomrule
    \label{sup_table:quan_extreme}
    \end{tabular}}    
\end{table}


==> supple_tex/D.3.HDR_metric.tex <==
\subsection{Comparison of reconstructed HDR to HDR GT}
% We report the updated version of the HDR-VDP metric~\cite{HDR-VDP-2}, which ranges in $[0,10]$, and follow the normalization~\cite{liu_single-image_2020} to deal with scale-ambiguity with our HDR results.
% Ours achieves 4.29$\pm$1.81 while ADOP achieves 3.97$\pm$1.72.
% Ours learns high-quality HDR results compared to ADOP.
% Our model can also produce more accurate results in HDR image rendering compared to ADOP.
To quantify the exactness of the HDR rendering, we adopt the HDR-VDP metric~\cite{HDR-VDP-2}.
We employ an updated version of HDR-VDP, which ranges in $[0,10]$ and follow the normalization~\cite{liu_single-image_2020} to deal with scale-ambiguity with our HDR results.
We measured HDR-VDP on all of our synthetic data.
Ours achieves 4.29$\pm$1.81 while ADOP achieves 3.97$\pm$1.72.
HDR-Plenoxels can learn precise results not only in LDR but also in HDR rendering.
